Vision-Centric BEV Perception: A Survey

In recent years, vision-centric Bird's Eye View (BEV) perception has garnered significant interest from both industry and academia due to its inherent advantages, such as providing an intuitive representation of the world and being conducive to data fusion. The rapid advancements in deep learning have led to the proposal of numerous methods for addressing vision-centric BEV perception challenges. However, there has been no recent survey encompassing this novel and burgeoning research field. To catalyze future research, this paper presents a comprehensive survey of the latest developments in vision-centric BEV perception and its extensions. It compiles and organizes up-to-date knowledge, offering a systematic review and summary of prevalent algorithms. Additionally, the paper provides in-depth analyses and comparative results on various BEV perception tasks, facilitating the evaluation of future works and sparking new research directions. Furthermore, the paper discusses and shares valuable empirical implementation details to aid in the advancement of related algorithms.

==> bio.tex <==
\newpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{MYX.jpg}}]{Yuexin Ma} received the PhD degree from the Department of Computer Science at University of Hong Kong in 2019.
Now she is an assistant professor in ShanghaiTech university, China, leading 4DV Lab. Her research interests lie on the computer vision and deep learning. Particularly she is interested in 3D scene understanding, multi-modal perception, human-machine cooperation, and autonomous driving. 
\end{IEEEbiography}




\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{wt.jpg}}]{Tai Wang} received the BEng degree in information engineering from Zhejiang University, China, in 2019. He is currently a Ph.D. student of the Department of Information Engineering, the Chinese University of Hong Kong, supervised by Prof. Dahua Lin. His research interests focus on general 3D perception, including different modalities, tasks and scenarios. He is also interested in other extensive 3D vision research and their robotic applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bxy.jpg}}]{Xuyang BAI} received the Ph.D. degree in the Department of Computer Science and Engineering at the Hong Kong University of Science and Technology under the supervision of Prof. Chiew-Lan Tai. Before joining HKUST, he received a Bachelor degree in Electronic Information Science and Technology from Beijing Normal University in 2018. His primary research topic is about point cloud registration and LiDAR perception.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yht.jpg}}]{Huitong Yang} received the M.S. degree in optical engineering from Guangdong University of Technology, China, in 2022. Now he is a Research Assistant in ShanghaiTech University, China. Particularly he is interested in 3D perception for autonomous vehicles and scene understanding.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hyn.png}}]{Yuenan Hou} received the BEng degree in automation from Nanjing University, China, in 2017. He obtained the PhD degree from The Chinese University of Hong Kong, under the supervision of Prof. Chen Change Loy and Prof. Xiaoou Tang. Now he is a researcher in Shanghai AI Laboratory. His research interest includes 3D perception, model compression, lane detection and image generation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{wym.jpg}}]{Yaming Wang} received the Ph.D. degree in the Department of Electrical and Computer Engineering at the University of Maryland, College Park, USA, under the supervision of Prof. Larry S. Davis. Before joining UMD, he received a BEng degree in Electronic Information Science and Technology from Tsinghua University, China. His research topics are about 3D object detection and fine-grained object recognition.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yu_qiao.jpeg}}]{Yu Qiao} is a professor with Shanghai AI Laboratory. His research interests include computer vision, deep learning, and bioinformation. He has published more than 300 papers in international journals and conferences, including T-PAMI, IJCV, T-IP, T-SP, CVPR, ICCV etc. His H-index is 73, with 36,000 citations in Google scholar. He is a recipient of the distinguished paper award in AAAI 2021. His group achieved the first runner-up at the ImageNet Large Scale Visual Recognition Challenge 2015 in scene recognition, and the winner at the ActivityNet Large Scale Activity Recognition Challenge 2016 in video classification. He is an associate editor of Pattern Recognition, Neural Networks, and JVCI. He served as the program chair of IEEE ICIST 2014.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yrg.png}}]
{Ruigang Yang} received his Ph.D. degree from University of North Carolina at Chapel Hill and M.S degree from Columbia University. He is the CTO of Inceptio and a full professor of computer science at the University of Kentucky. He was the director of Robotics and Autonomous Driving Lab at Baidu Research. He has published over 130 papers, which, according to Google Scholar, has receive over 14000 citations with an H-index of 61. He has received a number of awards, including US NSF Career award in 2004 and the Deans Research Award at the University of Kentucky in 2013.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{dm2018-face}}]
{Dinesh Manocha} is currently a Paul Chrisman Iribe Professor Professor of computer science at the University of Maryland, College Park. He received his B.Tech. degree in computer science and engineering from the Indian Institute of Technology, Delhi in 1987; M.S. and Ph.D. in computer science at the University of California at Berkeley in 1990 and 1992, respectively. Manocha has supervised more than 45 MS and Ph.D. students. His research interests include geometric computing, interactive computer graphics, physics-based simulation and robotics. 
%He has published more than 280 papers in these areas.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{zxg.jpeg}}]{Xinge Zhu} received the PhD degree in The Chinese University of Hong Kong under the supervision of Professor Dahua Lin, and the BEng degree in computer science from Shandong University, China. His research interests lie on the computer vision and machine learning. Particularly he is interested in 3D perception for autonomous vehicles, including 3D detection and 3D segmentation. He has published over 30 papers and received a number of awards, including multiple champions of open challenges, Waymo, NuScenes, etc.
\end{IEEEbiography}

==> futurework.tex <==
\section{Future Work}
